Quantum Model Learning Agent: characterisation of quantum systems through machine learning

Accurate models of real quantum systems are important for investigating their behaviour, yet are difficult to distill empirically. Here, we report an algorithm -- the Quantum Model Learning Agent (QMLA) -- to reverse engineer Hamiltonian descriptions of a target system. We test the performance of QMLA on a number of simulated experiments, demonstrating several mechanisms for the design of candidate Hamiltonian models and simultaneously entertaining numerous hypotheses about the nature of the physical interactions governing the system under study. QMLA is shown to identify the true model in the majority of instances, when provided with limited a priori information, and control of the experimental setup. Our protocol can explore Ising, Heisenberg and Hubbard families of models in parallel, reliably identifying the family which best describes the system dynamics. We demonstrate QMLA operating on large model spaces by incorporating a genetic algorithm to formulate new hypothetical models. The selection of models whose features propagate to the next generation is based upon an objective function inspired by the Elo rating scheme, typically used to rate competitors in games such as chess and football. In all instances, our protocol finds models that exhibit $F_1$-score $\geq 0.88$ when compared with the true model, and it precisely identifies the true model in 72% of cases, whilst exploring a space of over $250,000$ potential models. By testing which interactions actually occur in the target system, QMLA is a viable tool for both the exploration of fundamental physics and the characterisation and calibration of quantum devices.

==> content/todo.tex <==
\section*{To do list}
\begin{easylist}[itemize]
    % & \raf{We need to clarify why the F1 score is relevant and how we use it. Usually is used in classification}
    % && \raf{can we say anything about the connection between F1 Score and predictive power}
    % && \brian{please see if you think the new appdx section addresses this well enough: \cref{sm:f_score_justification}}
    % &&& I added a sentence at the end of p5 linking to it
    % & \raf{Missing information on the true models used}
    %     && \brian{I listed the true model for gen alg. please check if there's anything else missing and delete this bullet if you're happy }
    & \raf{Introduction and Abstract need a bit of work but there is where Nathan and Anthony could help considerably.}
    & \raf{can we change the formatting to a standard PRL style please? Place the todo list at the end etc. ? Also I think there are some improvements that could speed up working with this. e.g. get rid of useless files and correct file names)}
    & \raf{missing literature}
    && \brian{please add any papers I've missed}
    && \raf{Andrea I started adding something can you help adding also some of the other ones? Also arxiv references should be replaced with the published paper}
    && \andreas{OK, have started putting something on spot in the discussion but will have another check}
    & \raf{Problem of sampling, maybe solved by Arnuchalan}
    && \brian{you mean "Sample-efficient learning of quantum many-body systems"? sure - please     add reference where you think most appropriate}
    & \brian{@Raf @Anreas can you please both have a go at improving the discussion? I wrote something pretty generic that you can probably improve}
    && \andreas{I have started massaging and expanding a bit, but probably needs another go}
\end{easylist}

==> figure_development/obj_fnc_table.tex <==
\begin{tabular}{|cc|c|c|c|c|c|c|}
\hline
          &      &                              $\hat{H}_a$ &                              $\hat{H}_b$ &                              $\hat{H}_c$ &                              $\hat{H}_d$ &                              $\hat{H}_e$ &                              $\hat{H}_f$ \\
Method &  &                                          &                                          &                                          &                                          &                                          &                                          \\

          & $F_1$ &                                    $0.0$ &                                    $0.2$ &                                    $0.4$ &                                    $0.5$ &                                    $0.7$ &                                    $0.8$ \\
          & $k$ &                                        3 &                                        4 &                                        5 &                                        7 &                                        6 &                                        7 \\
          & $\overline{l_e}$ &                          $0.86 \pm 0.29$ &                          $0.84 \pm 0.29$ &                          $0.77 \pm 0.27$ &                          $0.78 \pm 0.29$ &                          $0.79 \pm 0.26$ &                          $0.79 \pm 0.26$ \\
          & $\tll_i$ &                                     -143 &                                     -152 &                                     -131 &                                     -150 &                                     -125 &                                     -124 \\
\hline \multirow{2}{*}{Inverse log-likelihood} & $g_i^L$ &                                  0.00698 &                                  0.00659 &                                  0.00766 &                                  0.00669 &                                  0.00803 &                                  0.00804 \\
          & $\%$ &                                       23 &                                        0 &                                       25 &                                        0 &                                       26 &                                       26 \\
\cline{1-8}
\hline \multirow{5}{*}{Akaike Info Criterion} & AIC &                                      293 &                                      311 &                                      271 &                                      313 &                                      261 &                                      263 \\
          & AICc &                                      293 &                                      312 &                                      272 &                                      314 &                                      262 &                                      264 \\
          & $w_i^A$ &                                 1.81e-07 &                                  1.4e-11 &                                  0.00724 &                                 4.15e-12 &                                        1 &                                    0.334 \\
          & $g_i^A$ &                                 1.17e-05 &                                 1.03e-05 &                                 1.35e-05 &                                 1.01e-05 &                                 1.46e-05 &                                 1.43e-05 \\
          & $\%$ &                                       22 &                                        0 &                                       25 &                                        0 &                                       27 &                                       26 \\
\cline{1-8}
\hline \multirow{4}{*}{Bayesian Info Criterion} & BIC &                                      301 &                                      322 &                                      284 &                                      331 &                                      277 &                                      281 \\
          & $w_i^B$ &                                 5.49e-66 &                                 1.26e-70 &                                 1.97e-62 &                                 1.11e-72 &                                 8.43e-61 &                                 8.95e-62 \\
          & $g_i^B$ &                                 1.11e-05 &                                 9.65e-06 &                                 1.24e-05 &                                 9.11e-06 &                                 1.31e-05 &                                 1.27e-05 \\
          & $\%$ &                                       23 &                                        0 &                                       25 &                                        0 &                                       27 &                                       26 \\
\cline{1-8}
\hline \multirow{2}{*}{Bayes factor points} & $g_i^p$ &                                        0 &                                        2 &                                        3 &                                        2 &                                        3 &                                        5 \\
          & $\%$ &                                        0 &                                       13 &                                       20 &                                       13 &                                       20 &                                       33 \\
\cline{1-8}
\hline \multirow{3}{*}{Ranking points} & Ranking &                                        6 &                                        4 &                                        3 &                                        5 &                                        2 &                                        1 \\
          & $g_i^R$ &                                        0 &                                      0.1 &                                      0.2 &                                        0 &                                      0.3 &                                      0.4 \\
          & $\%$ &                                        0 &                                       10 &                                       20 &                                        0 &                                       30 &                                       40 \\
\cline{1-8}
\hline \multirow{3}{*}{Elo rating} & Rating &                                      909 &                                      944 &                                     1042 &                                     1007 &                                     1011 &                                     1084 \\
          & $g_i^E$ &                                        0 &                                       35 &                                      133 &                                       98 &                                      102 &                                      175 \\
          & $\%$ &                                        0 &                                        0 &                                       26 &                                       19 &                                       20 &                                       34 \\
\cline{1-8}
\hline \multirow{3}{*}{Residuals} & mean$\{\tilde{r_p^e}\}$ &                                    0.132 &                                    0.146 &                                    0.114 &                                    0.138 &                                   0.0858 &                                   0.0715 \\
          & $g_i^r$ &                                    0.753 &                                    0.729 &                                    0.785 &                                    0.743 &                                    0.836 &                                    0.862 \\
          & $\%$ &                                       23 &                                        0 &                                       24 &                                        0 &                                       26 &                                       27 \\
\hline
\end{tabular}

